MeshSDF: Differentiable Iso-Surface Extraction

Geometric Deep Learning has recently made striking progress with the advent of continuous Deep Implicit Fields. They allow for detailed modeling of watertight surfaces of arbitrary topology while not relying on a 3D Euclidean grid, resulting in a learnable parameterization that is not limited in resolution. Unfortunately, these methods are often not suitable for applications that require an explicit mesh-based surface representation because converting an implicit field to such a representation relies on the Marching Cubes algorithm, which cannot be differentiated with respect to the underlying implicit field. In this work, we remove this limitation and introduce a differentiable way to produce explicit surface mesh representations from Deep Signed Distance Functions. Our key insight is that by reasoning on how implicit field perturbations impact local surface geometry, one can ultimately differentiate the 3D location of surface samples with respect to the underlying deep implicit field. We exploit this to define MeshSDF, an end-to-end differentiable mesh representation which can vary its topology. We use two different applications to validate our theoretical insight: Single-View Reconstruction via Differentiable Rendering and Physically-Driven Shape Optimization. In both cases our differentiable parameterization gives us an edge over state-of-the-art algorithms.

==> figures/fig_dim.tex <==
\begin{wrapfigure}[12]{l}{50mm}
			\begin{overpic}[clip, trim=8.0cm 7cm 17cm 6.5cm,width=0.3\textwidth]{figures/fig_dim.pdf}
			\put(8,4){\small{$\{s = 0\} $}}
			\put(0,23){\small{$\{s +  \Delta s = 0\} $}}
			\put(67,23){$\mathbf p$}
			\put(64,39){$\mathbf n (\mathbf p)$}
			\put(41,52){$\mathbf p'$}
			\put(26,64){$\mathbf n (\mathbf p')$}
			\end{overpic}
		\caption{Geometric relation between local surface change $\Delta \mathbf p = \mathbf p' - \mathbf p$ and signed distance field perturbation  $\Delta s$.	\vspace{2.0cm}}
		\vspace{2.0cm}
		\label{fig:dim}
\end{wrapfigure}

==> figures/fig_svr.tex <==
\begin{figure}[t]
        \vspace{-8pt}
		\begin{center}
		%
			\begin{overpic}[clip, trim=0.0cm 14cm 0 0.5cm,width=1.0\textwidth]{figures/fig_svr_pdf.pdf}
			\put(6,14.5){\small{Input }}
			\put(15,14.5){\small{\textit{MeshSDF} Raw}}
			\put(35,14.5){\small{refinment iterations}}
			\put(60.5,15.5){\small{target}}
			\put(59,13.5){\small{silhouette}}
			\put(74,14.5){\small{\textit{MeshSDF} Refined}}
			\end{overpic}
		\end{center}
		\vspace{-8pt}
		\caption{\textbf{Shilouette-driven refinment.} (a) given an input image, we exploit the differentiability of \textit{MeshSDF} to refine the predicted surface so that to match target silhouette in image space through Differentiable Rasterization \cite{kato2018neural}. }
\label{fig:svr}
\vspace{-6pt}
\end{figure}

==> figures/optimization_full.tex <==
\begin{figure}[t]
		\vspace{0pt}
		\begin{center}
		%,grid,tics=5
			\begin{overpic}[clip, trim=2.5cm 7.0cm 2.0cm 0.0cm, width=\textwidth]{figures/optimization_full.png}
    			\put(50,6){\small{optimization}}
    			\put(50,19){\small{optimization}}
    			\put(50,32){\small{optimization}}
    			
    			\put(96, 36){\small{$p_{max}$}}
    			\put(96, 27){\small{$0$}}
    			\put(96, 19.5){\small{$p_{min}$}}
    			
    			\put(-3, 34){\small{(a)}}
    			\put(-3, 23){\small{(b)}}
    			\put(-3, 8){\small{(c)}}
    			
    			
    			\put(72, 43.5){\small{optimized shape}}
    			\put(18, 43.5){\small{initial shape}}
    			
    			\put(11, 41){\small{simulated $p$}}
    			\put(26, 41){\small{predicted $p$}}
    			\put(75, 41){\small{predicted $p$}}
			\end{overpic}
		\end{center}
		\vspace{-4mm}
\caption{\textbf{Drag minimization.} We start with three random ShapeNet cars and minimize our objective function $\mathcal{L}_{task}$ with respect to the latent vector $\bz$ that describes them. In the first column, we show the initial shape as seen from the side, front, and top with the colors representing the pressure field $p$ predicted by the network $g_\beta$. The intermediate columns depict intermediate stages of the minimization. The last column depicts the final result. Note that the car at the bottom initially has a spoiler, which the optimizer removes. In other words, it turns a surface of genus-1 into one of genus-0. This is reverse of what we did in Fig.~\ref{fig:sanity} and would have been just as hard to do with earlier techniques that require an explicit mesh representation.} 
\label{fig:cfd_optimization_full}
\end{figure}

\comment{

	
	     We visualize our full constrained drag minimization pipeline for different initial shapes.
	     On the left-most column, we illustrate the ground-truth pressure field on the initial shape as computed by OpenFoam. On its right, the one predicted by our differentiable emulator. In the middle we visualize optimization iterations. Finally, on the right-most column, we depict the optimized car shape together with the pressure field predicted by the emulator.
	     Observe that, for the minimization in (c), we start with a shape with a spoiler (genus-1) and end up with a more aerodynamic car with different topology (genus-0).
	     This change of topology could not have been possible using \textit{classical} explicit surface parameterizations \cite{Baque18, Umetani18}. \ER{Switching to Figure with comparison to  \cite{Baque18, Umetani18}!!!}
	     
	     }
